A First Look at GPT Apps: Landscape and Vulnerability

Following OpenAI's introduction of GPTs, a surge in GPT apps has led to the launch of dedicated LLM app stores. Nevertheless, given its debut, there is a lack of sufficient understanding of this new ecosystem. To fill this gap, this paper presents a first comprehensive longitudinal (5-month) study of the evolution, landscape, and vulnerability of the emerging LLM app ecosystem, focusing on two GPT app stores: \textit{GPTStore.AI} and the official \textit{OpenAI GPT Store}. Specifically, we develop two automated tools and a TriLevel configuration extraction strategy to efficiently gather metadata (\ie names, creators, descriptions, \etc) and user feedback for all GPT apps across these two stores, as well as configurations (\ie system prompts, knowledge files, and APIs) for the top 10,000 popular apps. Our extensive analysis reveals: (1) the user enthusiasm for GPT apps consistently rises, whereas creator interest plateaus within three months of GPTs' launch; (2) nearly 90\% system prompts can be easily accessed due to widespread failure to secure GPT app configurations, leading to considerable plagiarism and duplication among apps. Our findings highlight the necessity of enhancing the LLM app ecosystem by the app stores, creators, and users.

==> Section/06_Recommendation.tex <==
\section{Recommendation}
Based on our findings, we provide some recommendations for users, creators, and app stores to improve the LLM app ecosystem.

\textbf{GPT App Users.}
Unlike traditional mobile apps that often provide detailed textual descriptions, UI designs, and screenshots to illustrate their functionality, many GPT apps lack comprehensive use-case descriptions that clarify what inputs produce specific outputs.
Therefore, user ratings and feedback become crucial, especially in the initial stages of GPT stores and apps, as they guide potential users in making informed choices about which apps to use. We suggest users can actively provide user ratings.

\textbf{GPT app creators.}
GPT app creators should be aware of the vulnerabilities inherent in GPT apps and make the protection of their configurations a priority. Given greater difficulties in acquiring external APIs, creators can transfer sensitive data to these APIs to prevent potential data leaks. Additionally, incorporating protective instructions within system prompts can further complicate unauthorized access to these prompts, enhancing security.

\textbf{GPT app stores.}
App stores serve as crucial intermediaries between creators and users, playing a vital role in the development of the app market and ecosystem.  From the perspective of dynamics and evolution, app stores could implement tangible incentives to foster engagement from both creators and users. Encouraging users to submit ratings and comments can facilitate the continuous development and refinement of apps. Similarly, providing financial incentives can spur creators' creativity and innovation, motivating them to explore new ideas and enhance the functionality of their apps.

From the security side, app stores should implement robust measures to safeguard the integrity and privacy of the apps they host. For example, they could set restricted review processes to screen apps for vulnerabilities and potential security risks and conduct continuous monitoring to detect and respond to threats promptly. Additionally, implementing strict data protection protocols and security barriers can help prevent unauthorized access and data leaks, ensuring a safe and secure environment for both users and developers. These practices are crucial for maintaining user trust and fostering a secure and sustainable app ecosystem.



% OpenAI's GPT app store is the official platform for displaying and retrieving GPT apps.
% Since all GPT app configurations submitted by creators are transparent to GPT app stores, it is essential to design appropriate monitoring mechanisms to enhance the protection of GPT apps, especially given the prevalence of plagiarism or duplication we observed.
% For example, the GPT store could alert GPT app creators to potential configuration leakage and apply stricter review phases for new GPT apps that likely plagiarize popular predecessors.
% They can also add an additional layer that filters potential sensitive user behavior and generated content during the conversation, like Cloudflare AI Firewall~\cite{cloudflare-ai-firewall}.
% These approaches could extend the sustainable development of the GPT app ecosystem.
% Moreover, providing financial incentives is imperative to attract more creators and ensure continuous development.

==> Section/Others.tex <==
\section*{Limitations}

This study mainly targets reverse-engineering GPTs via prompt attacks.
Yet, the protection of GPTs represents a crucial area for further investigation.
For instance, the investigation of GPTs with protection designs that have been successfully reverse-engineered in Level 2 and Level 3 attacks, as discussed in Section~\ref{sec:reverse-engineering}, is valuable.
Furthermore, exploring GPTs that require the creation of context-aware prompts to reveal their internals is also a promising direction.

\section*{Ethics Statement}
Our methodology involves using the web scraping tool. However, we just capture public web pages, with no privacy or sensitive information included. Furthermore, all the reverse engineering experiments are conducted under the restriction of the OpenAI quota.

% \section*{Acknowledgements}

